There and Back Again: Learning to Simulate Radar Data for Real-World Applications

Simulating realistic radar data has the potential to significantly accelerate the development of data-driven approaches to radar processing. However, it is fraught with difficulty due to the notoriously complex image formation process. Here we propose to learn a radar sensor model capable of synthesising faithful radar observations based on simulated elevation maps. In particular, we adopt an adversarial approach to learning a forward sensor model from unaligned radar examples. In addition, modelling the backward model encourages the output to remain aligned to the world state through a cyclical consistency criterion. The backward model is further constrained to predict elevation maps from real radar data that are grounded by partial measurements obtained from corresponding lidar scans. Both models are trained in a joint optimisation. We demonstrate the efficacy of our approach by evaluating a down-stream segmentation model trained purely on simulated data in a real-world deployment. This achieves performance within four percentage points of the same model trained entirely on real data.

==> 2-related-work_old.tex <==
\section{Related Work}
\subsection{Radar}

\subsection{Simulation}

\subsection{Radar Sensor Modelling}
Simulating radar sensor modelling is not a new problem with research interest spanning several decades. In the simplest approaches object lists (as returned by most commercial radars used in industry) can be approximated by querying the point locations and velocities of vehicles. In order to make simulation more realistic phenomological models can be used to account for clutter, limited resolution, angular sensitivity of the radar cross section and interference \cite{buhren2006simulation, buhren2007extension, buhren2007simulation},  

\subsection{Domain Transfer}
